Hierarchy construction schemes within the Scale set framework

Segmentation algorithms based on an energy minimisation framework often depend on a scale parameter which balances a fit to data and a regularising term. Irregular pyramids are defined as a stack of graphs successively reduced. Within this framework, the scale is often defined implicitly as the height in the pyramid. However, each level of an irregular pyramid can not usually be readily associated to the global optimum of an energy or a global criterion on the base level graph. This last drawback is addressed by the scale set framework designed by Guigues. The methods designed by this author allow to build a hierarchy and to design cuts within this hierarchy which globally minimise an energy. This paper studies the influence of the construction scheme of the initial hierarchy on the resulting optimal cuts. We propose one sequential and one parallel method with two variations within both. Our sequential methods provide partitions near the global optima while parallel methods require less execution times than the sequential method of Guigues even on sequential machines.

==> bounds.tex <==
\begin{picture}(0,0)%
\includegraphics{bounds.ps}%
\end{picture}%
\setlength{\unitlength}{4144sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(742,741)(1296,-1195)
\end{picture}%


==> kheops.tex <==

\begin{figure}[h!]

\centering

 \begin{tabular}{cc}

 \begin{tabular}{cccccc}


\begin{minipage}[b]{0.1\linewidth}
  MM
  \\
  \vspace{4mm}
\end{minipage}
&  \includegraphics[width=0.17\linewidth]{RES/kheops.eps}&  \includegraphics[width=0.17\linewidth]{RES/kheops/MIES/seg_cutBlack.eps} & \includegraphics[width=0.17\linewidth]{RES/kheops/MIES/seg_cutBlack20.eps} & \includegraphics[width=0.17\linewidth]{RES/kheops/MIES/seg_cutBlack12.eps}& \includegraphics[width=0.17\linewidth]{RES/kheops/MIES/seg_cutBlack05.eps}\\

 
\begin{minipage}[b]{0.1\linewidth}
  $MM^1$
  \\
  \vspace{4mm}
\end{minipage} 
& \includegraphics[width=0.17\linewidth]{RES/kheops.eps}&  \includegraphics[width=0.17\linewidth]{RES/kheops/multi/seg_cutBlack.eps} & \includegraphics[width=0.17\linewidth]{RES/kheops/multi/seg_cutBlack14.eps} & \includegraphics[width=0.17\linewidth]{RES/kheops/multi/seg_cutBlack08.eps}& \includegraphics[width=0.17\linewidth]{RES/kheops/multi/seg_cutBlack03.eps}\\

\begin{minipage}[b]{0.1\linewidth}
  $SM^2$
  \\
  \vspace{4mm}
\end{minipage}
&\includegraphics[width=0.17\linewidth]{RES/kheops.eps}&  \includegraphics[width=0.17\linewidth]{RES/kheops/n2/seg_cutBlack.eps} & \includegraphics[width=0.17\linewidth]{RES/kheops/n2/seg_cutBlack00.eps} & \includegraphics[width=0.17\linewidth]{RES/kheops/n2/seg_cutBlack10.eps}& \includegraphics[width=0.17\linewidth]{RES/kheops/n2/seg_cutBlack17.eps}\\

\begin{minipage}[b]{0.1\linewidth}
  SM
  \\
  \vspace{4mm}
\end{minipage}
&\includegraphics[width=0.17\linewidth]{RES/kheops.eps}&
\includegraphics[width=0.17\linewidth]{RES/kheops/nn/seg_cutBlack.eps}&
\includegraphics[width=0.17\linewidth]{RES/kheops/nn/seg_cutBlack00.eps} &
\includegraphics[width=0.17\linewidth]{RES/kheops/nn/seg_cutBlack08.eps}&
\includegraphics[width=0.17\linewidth]{RES/kheops/nn/seg_cutBlack17.eps}\\
\begin{minipage}[b]{0.1\linewidth}
  $SM^5$
  \\
  \vspace{4mm}
\end{minipage}&\includegraphics[width=0.17\linewidth]{RES/kheops.eps}&   \includegraphics[width=0.17\linewidth]{RES/kheops/n5/seg_cutBlack.eps} & \includegraphics[width=0.17\linewidth]{RES/kheops/n5/seg_cutBlack00.eps} & \includegraphics[width=0.17\linewidth]{RES/kheops/n5/seg_cutBlack10.eps}& \includegraphics[width=0.17\linewidth]{RES/kheops/n5/seg_cutBlack17.eps}\\


~&Image&$\lambda = 0.2$&$\lambda = 0.4$&$\lambda = 0.6$&$\lambda = 0.8$
\end{tabular}
&

\end{tabular}

\caption{\label{fig:kheops} partitions of pyramids image at
  different scales. Each line of the array corresponds to an heuristic
  whose acronym is indicated on the first column.}
\end{figure}


==> poubelle.tex <==
Conversely, given a
hierarchy $H$ and a value $\lambda$, each optimal cut of $H$ according to
$E_\lambda$ provides a partition of $I$ which is optimal among the set of
partitions which may be produced from $H$.  Paragraphs below show the
conditions that should be fullfilled by the energy terms of $E_\lambda$ in
order to define an unbiased multi-scale segmentation algorithm from
the sequence of optimal cuts. 


An unbiased multi-scale segmentation algorithm $P_\lambda$ will be called
\emph{optimal} according to an energy $E_\lambda$ and an image $I$, if
$E_\lambda(P_\lambda(I))$ is minimal among all the partition's energies produced
\emph{by unbiased multi-scale segmentation algorithms} for any value
of $\lambda$. 

The restriction by Guigues of the research space to a
hierarchy may thus be justified by the fact that the set of partitions
produced by optimal unbiased multi-scale segmentation algorithms
describes a hierarchy.  Note that the set $\mathbb{P}$ of partitions
on $I$ being finite, $H$ must be also finite.


This energy is roughly equal to the squared error of the image for
small values of $\lambda$ and encodes the global variation of the image.
The quantity may thus be interpreted as a normalised energy of optimal
cuts which varies between $0$ and $1$.

This normalisation allows to reduce the
influence of the global variation within an image and allows to
compare energies obtained on different images.

encoding In
this article, we have presented different heuristics for building
hierarchies on which optimal cuts according to an energy criterion may
be build.

These heuristics depict different compromizes between the energy of
the optimal partitions and the execution times.  We proposed one
sequential and one parallel method with two variations within both.
The method performing sequential merging , follows the scale-climbing
strategy proposed by Guigues but considers any subsets of the
neighborhood of each region. Bounding the cardinal of these subsets to
a suffiently high threshold allows to decrease the execution times
without altering significantly the quality of the output partitions.
The parallel merge algorithm is based on the notion of maximal
matching. We also proposed an alternative solution based on the basic
idea of the stochastic decimation process which consists to contract
at each step edges corresponding to a local minimum. This last
heuritic favors the energy criterion against the reduction factor.
Nevertheless all variations of the sequential method provide optimal
partitions with lower energies while both parallel decimation
processes run faster even on sequential computing machines. 



 such as
biomedical image processing \cite{leventon00level}, video image
analysis \cite{trivedi00distributed} and content-based image database
retrieval \cite{4761}.

Numerous approaches have been proposed to decompose an image into
meaningful regions. Within the region based approach methods based on
an homogeneity criterion have been early introduced. These methods
define a partition of an image into a minimal number of regions where
each region satisfies an homogeneity criteria. Top-down or bottom-up
segmentation methods respectively based on split and merge criteria
belong to this class.  These methods modify an initial partition by
split and/or merge operations until all the regions of the partition
satisfy a given criterion.  Note that, the homogeneity criterion is
often defined only implicitly since only the merge or split criteria
need to be defined.  Such an approach has been investigated by many
authors and recent bottom up methods combining new merge criteria and
an efficient ordering of the merge operations~\cite{} provide
interesting results.  Such methods allow to define the constraints
that each region of a partition should satisfy but do not readily
allow to define a global constraint on a partition.  This last
drawback is addressed by segmentation algorithms based on an energy
minimisation scheme.  Indeed, the energy of a partition provides a
criterion which should be globally minimized by segmentation
algorithms. Moreover, several segmentation algorithms based on a same
energy may be easily compared using the energy of the produced
partitions.

Energy based method are often defined from a criterion $D$ which
should be minimized over the partition. However, the direct
minimisation of $D$ often leads to a trivial solution. For example, if
$D$ corresponds to the distance to a piecewise constant image:
\[
D=\sum_{i=1}^nSE(R_i) \mbox{ with } SE(R_i)=\sum_{P\in R_i}\|I(p)-\mu_i\|^2
\]
the trivial solution made of one region $R_i$ for each pixel satisfies
$D=0$ and corresponds thus to a minimum. The term $\mu_i$ in the above
equation denotes the mean color or gray level of each region $R_i$.

Most of the energy based segmentation methods balance thus two terms
the criterion $D$ which encodes a fit to data and a criterion $C$
which may be interpreted as a regularisation term.  For example,
within the minimal cut /max flow framework~\cite{boykov-04} the energy
to be minimized can be represented as:
\[
E(P)=\sum_{p\in P} D_p(L_p) +\sum_{p,q\in \mathcal{N}}V_{p,q}(L_p,L_q)
\]
where $L=\{L_p, p\in I\}$ is a labeling of image $I$, $D_p(L_p)$ is a fit
to data term and $V_{p,q}(L_p,L_q)$ is an interaction potential
applied to each couple of adjacent pixels belonging to different
regions. This last term may be interpreted as a regularization term.



Comparing the parallel (SD) algorithm in Fig~\ref{fig:2a2}(L2) with sequencial one ($SM^2$) in Fig~\ref{fig:2a2}(L3) shows that results are quiet similar for any scale parameter. We can notice that parallel method tend to merge faster the biggest uniform regions. Nevertheless, Fig~\ref{fig:2a2}.(h) shows that mean energy for ($SM^2$) is smaller than for (MM) which merge at each step all local minima where ($SM^2$) merge only the global minimum.Fig~\ref{fig:2a2}.(h)  shows that both parallel methods run faster than sequential one even on sequential machines.\\

On the one hand, Fig~\ref{fig:2a2}.(g) shows that energy of partition for ($SM^{\infty}$) is lower than for ($SM^2$). Fig~\ref{fig:2a2} illustrates the fact that allowing multi-merging operations (Section~\ref{sec:MultiFusion}) can help to make  better choices during the decimation process.
For example, the stem of the mushroom is then, better captured in Fig~\ref{fig:2a2}(L4) with ($SM^{\infty}$) than in Fig~\ref{fig:2a2}.(L3) with ($SM^2$).
On the other hand Fig~\ref{fig:2a2}.(h) shows that the execution time for ($SM^{\infty}$) is bigger than for ($SM^2$).
Nevertheless, Fig~\ref{fig:2a2}.(g) shows that bounding by 5  the cardinal of the subsets $W \in \mathcal{P}(R) $ of the possible merging of a region with its neighbors don't alter significantly the energy of the optimal cuts. Fig~\ref{fig:2a2}(L5) shows that the quality of the results is quiet the same with ($SM^5$) thah with ($SM^{\infty}$) in Fig~\ref{fig:2a2}(L5) and we can just observe  that the boudaries are more regular without bounding $W$ (Fig~\ref{fig:2a2}.(L5)).\\



for each heuristic $h$ and for each value
of $\lambda$, the mean value:
\[
\frac{1}{N}\sum_{i=1}^N\frac{E_\lambda(C^*_\lambda(H_h^i))}{E_\lambda(P^i_{max})
\]
where $H_h^i$ denotes the hierarchy built by heuristic $h$ on image
$I_i$, $P^i_{max}$ encodes the partition and $E_\lambda(P
computed over all the image of the Berkley database.

  computed over
  the $100$ images of the database.

Given an image $I_i$ of the berkley database, a method $m\in
\{MM,MM^1,SM,SM^2,SM^5\}$ and a scale value $\lambda$, let us consider the
hierarchy $H^i_h$ produced by the heuristic $h$ on $I_i$ and the
quantity $E_\lambda(C^*_\lambda(H^i_h))$ which represents the energy of the
optimal cut within $H^i_h$ for this value of $\lambda$. Given, $h$ and $\lambda$
the quantity $E_\lambda(C^*_\lambda(H^i_h))$ may varry according to the image
content.  In order to reduce the influence of the global variation of
the image we propose to normalise the energy of each optimal cut by
the energy of the coarser optimal cut $P_{max}$ at a same $\lambda$. Due to
the sub additivity of $C$, $P_{max}$ corresponds to a single region
encoding the whole image. Its associated energy is equal to
$E_\lambda(P_{max})=SE(I)+\lambda|\delta(I)|$, where  Since
$E_\lambda(C^*_\lambda(H^i_h))$ is a piecewise linear concave function of $\lambda$, it
is located below the line associated to the interval $[\lambda_{max},+\infty)$.
The quantity $\frac{E_\lambda(C^*_\lambda(H^i_h))}{E_\lambda(P_{max})}$ belongs thus to
the interval $[0,1]$.



%The edges with minimum scale of appearance are then mark as \textit{member} of the set as follows.

%\begin{itemize}
%\item (1) Mark every edges $e \in E$ as \textit{candidate}.
%\item (2) do \begin{itemize}
%	\item (a) Assign scale of appearance $\lambda^+$ to the candidates of $E$
%	\item (b) Determine the candidates whose $\lambda^+$ is lower than the $\lambda^+$ of all neighboring candidates and mark them as \textit{member} (of the $MaIES$ ) and as \textit{non-candidate}. Also mark every neighbor of every new member as non-candidate.
%	\end{itemize}
%\end{itemize}

 The second heuristic we used is based on a parallel decimation
process. At each step we build a \textit{maximal edge sets} or
\textit{matchings}, set in which no pair of edges has a common vertex.
This \textit{edge sets} is maximal if we can't add any edge without
losing \textit{matching} property.
The maximal edge matchings  problem is solved iteratively. The  number of iterations to complete maximal independent set converges in most of the cases very fast \cite{meer89}. This set corresponds to the first step used by Haxhimusa \cite{haxhimusa03constructing} to build a Maximum Independent Directed Edge Set.\\
Let $V$ and $E$ denote the vertex set and the edge set of a graph
$G=(V,E)$, respectively and let $\iota(.)$ be the mapping from an edge to
its set of end vertices. The neighborhood $\Gamma(e)$ of an edge $e \in E$ is
defined by

$$$$

%$\alpha \beta \gamma \delta \epsilon \varepsilon \zeta \eta \theta \vartheta \iota \kappa \lambda \mu \nu \xi \pi \varpi\rho \varrho \sigma \varsigma \tau \upsilon \phi \varphi \chi\psi \omega \Gamma \Delta \Theta \Lambda \Xi \Pi \Sigma \Upsilon \Phi \Psi\Omega$ 

A maximal edge matching may be generated as follows

\begin{algorithm}[h!]
\caption{Maximal Edge Matchings Algorithm}
\begin{itemize}
\item (1) Mark every edges $e \in E$ as \textit{candidate}.
\item (2) Iterate the following two steps as long as there are candidates : 
	\begin{itemize}
	\item (a) Assign scale of appearance $\lambda^+$ to the candidates of $E$
	\item (b) Determine the candidates whose $\lambda^+$ is lower than the $\lambda^+$ of all neighboring candidates and mark them as \textit{member} (of the set ) and as \textit{non-candidate}. Also mark every neighbor of every new member as non-candidate.
	\end{itemize}
\end{itemize}
\label{algo1}
\end{algorithm}

\begin{figure}[h!]
\centering
\begin{tabular}{ccc}
\subfigure[]{
\label{fig:MISa}
\includegraphics[width=0.3\linewidth]{figures/MIS/MISa.eps}}&
\subfigure[]{
\label{fig:MISa2}
\includegraphics[width=0.3\linewidth]{figures/MIS/MISa2.eps}}&
\subfigure[]{
\label{fig:MISa3}
\includegraphics[width=0.3\linewidth]{figures/MIS/MISa3.eps}}\\
initial graph $G=(V,E) $& first iteration & second iteration 
\end{tabular}
  \caption{\label{fig:AlgoPara} The two iterations needed to obtain a maximal edge machings from graph $G$ }
\end{figure}

\subsection{Initial segmentation influence}

\begin{figure}[h!]
 \begin{tabular}{ccccc}
\subfigure[Image ]{
   \includegraphics[width=0.16\linewidth]{RES/sansLPE/model.eps}} &
\subfigure[ 0.2]{
\includegraphics[width=0.16\linewidth]{RES/sansLPE/seg_cutBlack00.eps}} &
\subfigure[0.4 ]{
 \includegraphics[width=0.16\linewidth]{RES/sansLPE/seg_cutBlack05.eps}} &
\subfigure[0.6 ]{
 \includegraphics[width=0.16\linewidth]{RES/sansLPE/seg_cutBlack12.eps}}&
\subfigure[0.8 ]{
 \includegraphics[width=0.16\linewidth]{RES/sansLPE/seg_cutBlack17.eps}}\\

  \end{tabular}


  \begin{tabular}{ccccc}
\subfigure[Image]{
   \includegraphics[width=0.16\linewidth]{RES/avecLPE/model.eps}} &
\subfigure[$ 0.2$]{
\includegraphics[width=0.16\linewidth]{RES/avecLPE/seg_cutBlack00.eps}} &
\subfigure[$ 0.4$]{
 \includegraphics[width=0.16\linewidth]{RES/avecLPE/seg_cutBlack05.eps}} &
\subfigure[$ 0.6$]{
 \includegraphics[width=0.16\linewidth]{RES/avecLPE/seg_cutBlack12.eps}}&
\subfigure[$ 0.8$]{
 \includegraphics[width=0.16\linewidth]{RES/avecLPE/seg_cutBlack17.eps}} \\
  \end{tabular} 

\caption{\label{fig:watershed} Optimal cuts, at different scale, in the hierarchy, starting from the pixels grid (b,c,d,e) and from a watershed segmentation (g,h,i,j).}
\end{figure}



Fig~\ref{fig:watershed}. shows the influence of the watershed used as initial segmentation on Barbara. Although the results are rather different in small scale, they are very similar in the coarser level. The energies $E_{\lambda}(P)$ obtained with or without watershed segmentation are also very similar (Fig~\ref{fig:lpeNRJ}).
The algorithm is then very stable as soon as initial the pixels grid segmentation is composed of as many regions as over-segmentation, obtained with the watershed algorithm.

 As  we can see in Fig~\ref{fig:1a1}. the time needed to build the hierarchy is commensurate with the number of regions in the initial segmentation.
Hence, starting from the pixels grid weighty increases the processing time and contributes to  lead to a lower energy. We can see in Fig~\ref{fig:lpeNRJ}. that energies obtain without watershed are just a little lower.

Starting from a watershed segmentation seems to be a good option that can speed up by ten the application, and gives almost the same energy for any scale parameter.


\begin{figure}
\includegraphics[width=0.4\linewidth]{RES/lpeNRJ.eps}
\caption{\label{fig:lpeNRJ} energy  $E_{\lambda}(P)$ for a hierarchy starting from a watershed segmentation(red) and from the pixels grid (blue)}
\end{figure}

\begin{figure}[h!]
\begin{tabular}{cccc}
\includegraphics[width=0.2\linewidth]{img/RAGnum.eps}
\includegraphics[width=0.2\linewidth]{img/para3.eps}
\includegraphics[width=0.2\linewidth]{img/para3d.eps}
\includegraphics[width=0.2\linewidth]{img/para7.eps}
%  \caption{\label{fig:AlgoPara} }
\end{tabular}


\end{figure}



 For every $R_i$ in $P_0$, all the grouping including $R_i$
and its neighboring combinations are considered. The number of
combinations is then given by $\sum_{j=1}^{n_b}C_{n_b}^{j} = 2^{n_b -
  1}$ with $C_{n_b}^{j}$ being the number of combinations of $j$
neighbors among $n_b$. This approach includes the Guigues'method which
allows to merge only two adjacent regions. Hence, if a grouping is
composed of two regions,with the minimum scale of appearance, it will
be selected and merge.

 


\begin{figure}[h!]
\begin{tabular}{cccccc}

\includegraphics[width=0.2\linewidth]{img/multi1.eps} &
\includegraphics[width=0.2\linewidth]{img/multi2.eps} &
\includegraphics[width=0.2\linewidth]{img/multi4.eps} &
\includegraphics[width=0.2\linewidth]{img/multi5.eps} &
\includegraphics[width=0.2\linewidth]{img/multi7.eps}  \\
  \end{tabular}
 \caption{\label{fig:Algomulti}5 of the 7 different grouping including region A and its  neighboring combinations } 
\end{figure}

Despite these theoritical justifications, the energy described by
equation~\ref{eq:mumford} combines two terms wich are not homogeneous.
Indeed, the squared error is proportional to a surface while the
second term is proportional to a length. This lack of homogneity,
leads to a total energy for each region which is largely dominated by
the squared error except for very high values of $\lambda$. This last
drawback induces unbounded values $\lambda^+(R)$ for the scale of
appearance of the different regions. Therefore, we propose to use a
nomalize energy defined by:
\begin{equation}
  E^{mum}_\lambda(P)=D(P)+\lambda C(P)=\sum_{i=1}^n\frac{SE(R_i)}{\sum_{i=1}^nSE(R_i)}+\lambda\frac{|\delta(R_i)|}{|I|}\label{eq:normal}
\end{equation}
where each term $\frac{SE(R_i)}{\sum_{i=1}^nSE(R_i)}$ corresponds to a
measure of the relative weight of a region compared to the total
homogeneity of its partition. This measure is bounded by the values
$0$ and $1$.  The term $|I|$ measures the total length of the image
boundary $2(H+W)$ where $H$ and $W$ denote the height and width of the
image.  While we can not insure that $\frac{|\delta(R_i)|}{|I|}$ is
always lower than $1$, the normalisation of the region boundaries by
the length of the image boundaries improves the normalisation of
the scale of appearances to 

 More formally, our fit to data term for
each region $R_i$ of a partition is defined as:
\[
D(R_i)=\frac{SE(R_i)}{\sum_{i=1}^nSE(R_i)}
\]
 instead ofenergy based
on squared errors tend at high levels of the hierarchy (i.e. for
coarse partitions) to mainly merge regions refuse merge operations

We consider affine separable energie, which can be written : \\

$E_{\lambda}(P)= \lambda C(P) + D(P)$

with the fitting term $D(R\in P) = \frac{SE(R)}{PE(P)}$ ( region squared error normalised with the partition error and the regularization term $ C(R)$ ( region boundaries length ).\\ 
\begin{tabular}{ll}
squared error : $SE(R) = \sum_{i \in R}||c_i - \mu_R ||^2$ & minimal if there is as many regions as pixels in the image   \\
partition error : $PE(P) =\sum_{R \in P} SE(R)$ & weak if there are few regions
 \end{tabular}

We choose to normalise the fitting term with partition error to avoid mixing terms relative to a surface and an other relative to boundaries.

Experimentaly, only using square error, give huge $\lambda$, and tend  to refuse to merge biggest regions. In this case, we can consider, the fitting term $D(R)$, as the global partition error involvement from the region $R$.



The energy used to describe a partition of an image into regions with
constant intensity and colors has been introduced by Leclerc~\cite{}
and Mumford and Shah~\cite{} in different frameworks. 



Moreover,
we observed during our experiments that for coarse partitions, when
the colorimetric distances between regions are roughly comparables,
the merge operations guided by the minimisation of
equation~\ref{eq:mumford} tend to merge all the small remaining
regions before merging largest ones. This last drawback may be
explained by the variation
\begin{equation}
  \Delta D^{mum}(P)=|R_2|\frac{x}{1+x}\|\mu_{R_1}-\mu_{R_2}\|^2\label{eq:deltaMum}
\end{equation}
of the term $D^{mum}(P)$ when we merge two regions $R_1$ and $R_2$
with $|R_1|<|R_2|$. The symbol $x$ represents the ratio
$\frac{|R_1|}{|R_2|}$. Equation~\ref{eq:deltaMum} tends to $0$ for
small values of $x$ independently of the mean colors of the regions.


We thus proposed to normalize the term $D^{mum}(P)$ by 


%\label{sec:States of the art}

%\subsection{Guigues}


%A low-level segmentation algorithm should not focus on a specific scale but rather on a multi-scale description of images. For example, in a region-oriented approach, this kind of description should be called a multi-scale segmentation.\\
%Those multi-scale segmentations can be represented exactly, considering a scale-sets representation.
%Guigues shows that one can build scale-sets whose sections approximate the solutions of a general energy minimization problem which embeds most %optimization-based formulations of the segmentation problem (variational, Markovian,
%minimal encoding). %The energies involved have two global terms whose relative weight is controlled by a real parameter $\lambda$ which, generally behaves %as a scale parameter. Guigues restricts the type of energies considered to what he call \textit{affine separable energies}, which are the energies which %can be written for partition P $$ E_{\lambda}(P)= \sum_{\mR \in P} \lambda C(P) + D(P) $$

Let $A(\lambda)$ a partitioning algorithm, whose result only depends on a parameter $\lambda \in \mR$. For a given image $I$, $A$ is said to be \textit{causal} if the partition returned by $A$ are ordered in $\lambda$, when
$$\lambda_1 \leq \lambda_2 \Longleftrightarrow A(\lambda_1) \leq A(\lambda_2)$$ where $\leq$ denote a partial order relation between partitions.
Intuitively $\lambda$  behaves as a scale parameter if increasing $\lambda$ systematically coarsens the partition produced. It can be derived from a fundamental principle of multi-scale analysis : the causality principle \cite{Koenderink84}. This principle says thas for any $\lambda_2 > \lambda_1$, the differents structures found at scale $\lambda_2$ should find a  \emph{cause} at scale  $\lambda_1$.

Let $P_{\lambda_i}$ be the partition of an image I, given by $A$($\lambda_i$) . In this case, for segmentation purpose, the parameter $\lambda$ behaves as a scale parameter if for $\lambda_2 > \lambda_1$,we can deduce the partition $P_{\lambda_1}$ from $P_{\lambda_2}$ by merging only some regions into larger units ($P_{\lambda_1}$ is coarser than $P_{\lambda_2}$  ).


%(the boundaries of partition $P_{\lambda_2}$ are in a one-to-one mapping with a subset of the boundaries of $P_{\lambda_1}$ ). 

All the resultats of A, when $\lambda$ browse $\mR^+$ give a set of partitions $\{P_{\lambda}\}_{\lambda \in \mR^+}={P_1 \leq P_2 \leq ... \leq P_3}$. The transition between $P_i$ and $P_{i+1}$ consists in merging some regions of $P_i$. Keeping only these merging events in the representation, give us a set of regions $H$ with a structure of hierarchy.

Hierarchies have a causal structure if the affine separable energy $$E_{\lambda}(P) = \sum_{R \in P} \lambda C(R) + D(R)$$ verifies some conditons.

 The goodness-of-fit term $D$ can be indifferent, but the regularising energie $C$ add to be subadditive :
$$\forall (R_1,R_2) \in P \Longleftrightarrow C(R_1 \cup R_2) \leq C_{R_1} + C_{R_2}$$

This is a natural condition, in segmentation task, as usual regularizing energies are decreasing. For example, quantifying the complexity of a segmentation by its number of regions, or summing up any positive quantity along the boundaries leads to decrease this kind of energy.\\

Guigues proposed to capture all the results of a partitioning  algorithm $P$ with respect to $\lambda$ into a single representation. For each $\lambda \in \mR^+$,  we call optimal $\lambda-cut$ the cut of $H$ who minimizes $E_{\lambda}$ and we denote this cut by $H_{lambda}$.
For any hierarchie $H$ with a causal structure, two regions of $H$ are either disjoint or nested. Considering the set of scales $\lambda$ for wich a region $R$ belongs to the optimal cut $H_{\lambda}$. Because of the causality of $H$, this set is an interval $[\lambda^+(R),\lambda^-(R)]$, with $\lambda^+(R)$ called scale of appearance and $\lambda^-(R)$ scale of disappearance of the region $R$. We can see that a region $R$ disappears when its father appears in a solution of $P$.

Hence, a couple $S=(H,\lambda^+)$, where $H$ is a hierarchy of regions and $\lambda^+ : H \to \mR^+$ is a fonction which provides the scale of appearance of the regions of H, can represente a complete result of a partitioning  algorithm $P$. It provides a scale-set representation of the multi-scale partitioning algorithm.


The partitions $\{P_{\lambda}\}_{\lambda \in \mR^+}$ are implicitely represented in S and can be retrieve by making \textit{cut} of the scale-sets (sets whose scale of appearance $\lambda^+$ is lower than $\lambda$ belongs to $P_{\lambda}$)

%\subsection{Minimal cuts in a hierarchie}

Guigues presents a fonctional dynamic procedure to compute $\lambda$ and $E_{\lambda}(R)$ for any $R$ in a hierarchy $H$. Considering only separable energie, which can be written $ E_{\lambda}(P)= \sum_{\mR \in P} \lambda C(P) + D(P)$, he provides a way to compute exactly  $\lambda^+(R)$ and $\lambda^-(R)$ by two runs in $H$: bottom-up then top-down. A bottom-up traversal of H allows to compute $ E_{\lambda}(R)$ and  $\lambda^+(R)$ for each region $R$. The top-down traversal allows to compute $\lambda^-(R)$.
Those two runs reveals regions which never belong to an optimal cut for $E_{\lambda}$ ( regions with  $\lambda^-(R) \leq \lambda^+(R)$). Such regions are removed from the initial herarchy, and we obtain a \textit{persistent hierarchy} for $E_{\lambda}$ (with $\lambda^+$ increasing from the leaves to the root of the tree).

%\subsection{Scale climbing}

The proposed strategy to construct the hierarchie itself is called \textit{scale climbing}. Starting from the base of the hierarchy it recursively adds in the representation the set that would first become optimal for $E_{\lambda}$ during a progressive increase of $\lambda$.

He consider building $H$ by a region merging strategy. Starting from an initial over-partition $P_0$, and after computing all the scale of appearance, the scale climbing algorithm chooses the pair of candidate whose scale of appearance is minimal (the region which demands the least regularization to become a solution). After $N-1$   climbing step (with $N$, the number of regions in over-partition $P_0$), the whole image is merged and a complete hierarchy $H$ has been built. After removing all region, with $\lambda^- \leq \lambda^+$, we obtain the persistent hierarchy $H^*$ and the \textit{scale climbing scale-set} $(H^*,\lambda^+)$.

An important property is that the structure ($H$) of a scale climbing scale-set is thus invariant by any linear transform on the energies considered. Hence, 
tuning the parameter $\lambda$ in the definition of the energies (a priori) or in the scale-sets (a posteriori) is equivalent.


 has in recent years, received a great deal of attention
whitin the Vision community.  Other methods like graph cuts
\cite{kolmogorov02what} and methods based on region merging scheme
have also been proposed \cite{2004SPIE}.

 The energies involved usually have two global terms whose relative weight is controlled by a real parameter $\lambda$ which, generally, behaves as a scale parameter. The type of energies considered are  most often \textit{affine separable energies}, which are the energies which can be written for partition P $$ E_{\lambda}(P)=  \lambda C(P) + D(P) $$

$E_\lambda(P)$ corresponds to the expression of a regularized ill-posed variational problem. $D$ is then usually called a fitting term and $C$ a regularization term widely use as encoding cost like in MDL theories to quantifie the complexity of a segmentation.
The \textit{scale parameter} $\lambda$ allows to browse a sequence of partitions and thus it controls the structural granularity.\\
%For segmentation purposes, the archetype of this kind of formulation is given by Mumford and Shah functional (Mumford and Shah, 1989).


Graph-cut approaches for Computer Vision have been particularily investigated by Yuri Boykov, Olga Veksler and Ramin Zabih \cite{boykov99fast}.
 A graph $G(V,E)$ can be partitioned into two disjoint sets( with $A\cup B=V$ et $A\cap B=\emptyset$) by simply removing edges connecting the two parts. The degree of dissimilarity between these two components can be computed as the weights of the edges that have been removed. 
 %In graph theoretic language, it is called the cut:  
$$cut(A,B) = \sum_{u\in A,v \in B}w(u,v) $$

The optimal bipartitioning of a graph is the one that minimizes this cut value. \cite{boykov97markov}
% There exist efficient algorithms for finding the minimum cut of a graph but
However, the minimum cut criteria favors cutting small sets of isolated nodes. To avoid this problem, Shi \& Malik \cite{shi00normalized} proposed to normalise this measure of disassociation :
% Instead of looking at the value of total edge weight connecting the two partitions, this measure computes the cut cost as a fraction of the total edge  onnections to all the nodes in the graph. This disassociation measure is called the normalized cut (Ncut):

$$Ncut(A,B) = \frac{ cut(A,B)}{assoc(A,V)} +\frac{ cut(A,B)}{assoc(B,V)}) $$
where $ assoc(A,V)= \sum_{u\in A,t \in V}w(u,t) $ is the total connection from nodes in $A$ to all nodes in the graph.
 With this new definition, $cut(A,B)$ can be considered as a fitting term and $assoc(A,V)$ acts  as a regularization term with which the cut that partitions out small isolated points will no longer have small Ncut value.\\

The level set method, for segmentation purpose, was first introduced by Osher and Sethian \cite{osher88fronts}. Over the years, the method has proven to be a robust numerical device for this purpose in a diverse collection of problem.


Level Sets are an implicit representation of a contour $C$ whose front is evolving with a signed distance fonction, $F$. Then, the set of values, for which the fonction $F$ is zero, represents the contour. This contour is evolving according to the  variations of a fonctionnal define on the image domaine.

Only two classes  can be represented, with conventional Level Set methods, but solutions for three and more classes are suggested. Zhao \cite{zhao96variational}  proposed to use a separate embedded surface for each class and Chan \& Vese) adopt a multi-phace evolution approch \cite{vese01multiphase}. Nevertheless all these approaches involve an a priori knowlegde on the number of regions.\\

A low-level segmentation algorithm should not focus on a specific scale but rather on a multi-scale description of images. For example, in a region-oriented approach, this kind of description should be called a multi-scale segmentation.
Guigues \cite{guigues03} proposed a new energy minimization framework for hierarchical segmentation, 
%based on an energy whose minimization defines a partition related to a given problem.
which explicits a scale parameter. This framework provides a continuous representation of the solutions according to a scale parameter, like in scale-space theories. 
For each value of the scale parameter, the method of Guigues provides the optimal solutions within a search-apace encoded as a hierarchy of regions.
 %The hierarchy of partitions  is explicitly encoded and the reduction scheme consists in merging at each step the two regions, whose merging involve the smallest increase in the energie.
 
Therefore, contrary to Level-Set or Graph-Cut/Ncut methods whose tend to find a local minimum in the whole search space, Guigues suggest tracking the global minimum in a restricted search-space. How can this narrow search-space, affect the stability of the segmentation algorithm, and what's it's influence on the final solutions ?\\
% of the partition based on the Mumford-Shah fonctionnal (citation).

We presents in section 2 the new energy minimization framework for hierarchical segmentation, proposed by Guigues, whose provides the optimal solutions within a search-apace. We proposed different heuristics to build such search-space in section 3. We then present in section 4 some experiments resultats.



%We propose to modify this framework  by adding the possibility, during the reduction process, of merging at each step 2,3 or more regions to limit the energy growth.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "gbr2007"
%%% End: 

